Decentralized Energy Marketplace via NFTs and AI-based Agents

The paper introduces an advanced Decentralized Energy Marketplace (DEM) integrating blockchain technology and artificial intelligence to manage energy exchanges among smart homes with energy storage systems. The proposed framework uses Non-Fungible Tokens (NFTs) to represent unique energy profiles in a transparent and secure trading environment. Leveraging Federated Deep Reinforcement Learning (FDRL), the system promotes collaborative and adaptive energy management strategies, maintaining user privacy. A notable innovation is the use of smart contracts, ensuring high efficiency and integrity in energy transactions. Extensive evaluations demonstrate the system's scalability and the effectiveness of the FDRL method in optimizing energy distribution. This research significantly contributes to developing sophisticated decentralized smart grid infrastructures. Our approach broadens potential blockchain and AI applications in sustainable energy systems and addresses incentive alignment and transparency challenges in traditional energy trading mechanisms. The implementation of this paper is publicly accessible at \url{https://github.com/RasoulNik/DEM}.

==> Figs/DEM-contracts-tikz.tex <==

\begin{tikzpicture}[scale=.7, transform shape,
    node distance = 2cm and 2cm, % set the horizontal and vertical distances
    auto,
    font=\footnotesize,
    user/.style={circle, draw=black!90, fill=green!20, thick, minimum size=0.5cm},
    nft/.style={rectangle, draw=blue!50, fill=blue!20, thick, minimum size=0.5cm},
    contract/.style={rectangle, draw=red!70, fill=red!20, thick, minimum size=1cm},
    contractBig/.style={rectangle, draw=red!70, fill=red!20, thick, minimum size=1.5cm},
    oracle/.style={ellipse, draw=black!90, fill=black!20, thick, minimum size=1cm},
    DEM/.style={rectangle, draw=black!70, fill=black!10, thick, minimum size=3cm},
    arrow/.style={->, >=stealth, thick, shorten <=1pt, shorten >=1pt},
    two-sided-arrow/.style={<->, >=stealth, thick, shorten <=1pt, shorten >=1pt, bend left=30}
]

% ... rest of your diagram ...
    % DEM
\node[DEM, label=above: {Decentralized Energy Market (DEM)}] (DEM) at (6, 3.5) {};

% Contracts
\node[contract, label=above: {EMarket}] (EMarket) at (9, 3.5) {
 \includegraphics[scale=0.07]{img.png}
};
\node[contractBig, label=above: {EPool}] (EPool) at (6, 3.5) {
\includegraphics[scale=0.05]{img.png}
};
\node[contract, label=above: {EP NFT}] (EP_NFT) at (3, 3.5) {
\includegraphics[scale=0.07]{img.png}
};
%
% Oracles
\node[oracle, label=below: {Energy Oracle}] (EnergyOracle) at (6,1) {};
\node[oracle, label=below: {Price Oracle}] (PriceOracle) at (9,1) {};


% Users and Grid Operator
\node[user, label=below: {User}] (User) at (0, 2) {};
\node[user, label=below: {Grid Operator}] (GridOperator) at (0, 4) {};
%
% Energy Profile NFTs
\node[nft,label=below:{\tiny NFT-user}] (NFT-user) at (5, 3.7) {};
\node[nft,label=below:{\tiny NFT-grid}] (NFT-grid) at (7, 3.7) {};



% Connections
\draw[arrow] (User) -- (EP_NFT);
\draw[arrow] (GridOperator) -- (EP_NFT);
\draw[two-sided-arrow] (EP_NFT) -- (EPool);
\draw[two-sided-arrow] (EPool) -- (EMarket);
\draw[arrow] (PriceOracle) -- (EMarket);
\draw[arrow] (EnergyOracle) -- (EPool);
\end{tikzpicture}




